Efficient Non-parametric Bayesian Hawkes Processes

In this paper, we develop an efficient nonparametric Bayesian estimation of the kernel function of Hawkes processes. The non-parametric Bayesian approach is important because it provides flexible Hawkes kernels and quantifies their uncertainty. Our method is based on the cluster representation of Hawkes processes. Utilizing the finite support assumption of the Hawkes process, we efficiently sample random branching structures and thus, we split the Hawkes process into clusters of Poisson processes. We derive two algorithms -- a block Gibbs sampler and a maximum a posteriori estimator based on expectation maximization -- and we show that our methods have a linear time complexity, both theoretically and empirically. On synthetic data, we show our methods to be able to infer flexible Hawkes triggering kernels. On two large-scale Twitter diffusion datasets, we show that our methods outperform the current state-of-the-art in goodness-of-fit and that the time complexity is linear in the size of the dataset. We also observe that on diffusions related to online videos, the learned kernels reflect the perceived longevity for different content types such as music or pets videos.

==> sections/introduction_backup.tex <==
%!TEX root = ../main.tex
%
\section{Introduction} 
\label{sec:introduction}

\begin{figure}[t] 
\centering
\subfloat[Poisson Cluster Process ]{{\includegraphics[scale=0.28, trim={8.5cm 2cm 9cm 2cm},clip]{hp_2_pps.pdf}}}
\subfloat[Branching Structure]{\raisebox{4ex}{\includegraphics[scale=0.35, trim={11cm 6cm 13cm 
4cm},clip]{branching_structure.pdf}}}
\caption{Cluster Representation of the Hawkes Process. (a) A Hawkes process with decaying triggering kernel $\phi(\cdot)$ has intensity $\lambda(t)$ which increases after each new point is generated. It can be represented as a cluster of Poisson processes PP($\phi(t-t_i)$) associated with each $t_i$. For the triggering relationships shown in (a), a  branching structure can be established as (b), where $t_1 \rightarrow t_3$ represents $t_1$ causes $t_3$ and $p_{31}$ is the probability of $t_3$ being generated by $t_1$.}
\label{fig:hp_2_pps}    
\end{figure}

The Hawkes process \citep{10.2307/2334319} is a useful model to describe self-exciting point data in which every point increases the likelihood of arrival of new points. More specifically, every point causes the conditional intensity function $\lambda(\cdot)$ which modulates the arrival rate of new points to increase. An alternative understanding of the Hawkes process is the Poisson cluster process \citep{10.2307/3212693} which categorizes points into \textit{immigrants} and \textit{offspring}.
Immigrant points are generated independently at a rate of $\mu(\cdot)$ and offspring points are triggered by existing points at a rate of $\phi(\cdot)$. Points are structured into clusters, associated with each immigrant point, which is called the branching structure (an example shown in \cref{fig:hp_2_pps}).

Many recent work employing Hawkes processes designs 
parametric background intensities and triggering kernels \citep{rizoiu2017expecting,Mishra2016FeaturePrediction,filimonov2015apparent,kurashima2018modeling,tabibian2017distilling,zhao2015seismic}. Manually designing parametric Hawkes models is an expensive process and may not generalize well to other applications. A typical solution to this problem is non-parametric estimations \citep{lewis2011nonparametric,zhou2013learning,eichler2017graphical,bacry2012non,bacry2014second, kirchner2017estimation} which are introduced in \cref{sec:non_parametric}. They are frequentist methods and there is few work on the non-parametric Bayesian estimation for the Hawkes process \citep{rousseau2018nonparametric}. The main difficulty to developing non-parametric Bayesian methods is $O(N^2)$ time taken to calculate the log-likelihood of the Hawkes process, where $N$ is the number of points.

In this paper, a general framework is proposed for the efficient non-parametric Bayesian inference of the Hawkes process. We exploit block Gibbs sampling \citep{ishwaran2001gibbs} to iteratively sample the latent branching structure, the background intensity $\mu(\cdot)$ and the triggering kernel $\phi(\cdot)$. In each iteration, point data are decomposed as a cluster of Poisson processes based on the sampled branching structure. All Poisson processes are aligned to estimate posterior $\mu$ and $\phi(\cdot)$. Our framework is close to the stochastic Expectation-Maximization (EM) algorithm \citep{celeux_diebolt85} where posterior $\mu(\cdot)$ and $\phi(\cdot)$ \citep{adams2009tractable, lloyd2015variational,samo2015scalable, pmlr-v70-walder17a, gugushvili2018fast} are estimated in the M-step and random samples of $\mu(\cdot)$ and $\phi(\cdot)$ are drawn.
Here, we assume $\mu(\cdot)$ is an unknown constant and the recent non-parametric Bayesian estimation for Poisson process intensities, termed Laplace Bayesian Poisson process (LBPP) \citep{pmlr-v70-walder17a}, is used to estimate the posterior $\phi(\cdot)$ given the sampled branching structure. Furthermore, the connection to the EM algorithm \citep{Dempster77maximumlikelihood} is explored and a variant of our method is proposed as an approximate EM algorithm. 
On synthetic data, we show our method can infer the exponential and the cosine triggering kernels, and the fitting time of our method is linear to the number of points. On real-life data our method outperforms the parametric Hawkes process (by 22\% and 12\% in the log-likelihood).

==> sections/related_work.tex <==
\section{Related Work}
This section introduces applications, variants and non-parametric estimations for Hawkes processes.

\subsection{Hawkes Processes}
The Hawkes process \citep{10.2307/2334319}, as a powerful tool to analyze the self-exciting phenomena in the real life event sequences, has been applied to a wide range of problems. \citet{Mishra2016FeaturePrediction} employ the branching factor of the Hawkes process to predict popularity of tweets;  \citet{kurashima2018modeling} predict human actions by the Hawkes process; information reliability and information source trustworthiness of online knowledge repositories are evaluated by the Hawkes process \citep{tabibian2017distilling}. Further evidence of the importance is that variants of the Hawkes process are proposed recently, such as HawkesN \citep{rizoiu2018sir}, which generalizes the Hawkes process accounting for a finite population size, Hawkes Intensity Processes \citep{rizoiu2017expecting}, modeling the expected Hawkes intensity, Isotonic Hawkes Processes \citep{wang2016isotonic}, nonlinear Hawkes processes.

\subsection{Non-parametric Estimation for the Hawkes Process}\label{sec:non_parametric}
There are situations where the shape of the suitable Hawkes triggering kernel is unknown, so the non-parametric estimation method is necessary. Recent methods include  EM algorithm based estimations \citep{lewis2011nonparametric,zhou2013learning},
 the least-squares-based learning
method \citep{eichler2017graphical}, the spectral-method-based estimation \citep{bacry2012non}, the Wiener-Hopf-based methods \citep{bacry2014second} and the integer-valued-autoregressive-model-based method  \citep{kirchner2017estimation}. These are frequentist methods and there has been much less work on Bayesian estimations for Hawkes processes. \citet{rasmussen2013bayesian} propose two Bayesian inference methods which approximate posterior distributions of Hawkes parameters by Markov chain Monte Carlo (MCMC). Most recently, \citet{rousseau2018nonparametric} exploits MCMC to estimate the posterior Hawkes model, which is closest to our method. The main difference is that our work uses the stochastic branching structure to accelerate the estimation of the posterior Hawkes process.
